Luttinger's theorem, superfluid vortices, and holography

Strongly coupled field theories with gravity duals can be placed at finite density in two ways: electric field flux emanating from behind a horizon, or bulk charged fields outside of the horizon that explicitly source the density. We discuss field-theoretical observables that are sensitive to this distinction. If the charged fields are fermionic, we discuss a modified Luttinger's theorem that holds for holographic systems, in which the sum of boundary theory Fermi surfaces counts only the charge outside of the horizon. If the charged fields are bosonic, we show that the the resulting superfluid phase may be characterized by the coefficient of the transverse Magnus force on a moving superfluid vortex, which again is sensitive only to the charge outside of the horizon. For holographic systems these observables provide a field-theoretical way to distinguish how much charge is held by a dual horizon, but they may be useful in more general contexts as measures of deconfined (i.e. "fractionalized") charge degrees of freedom.

==> revcomments <==
We certainly agree with the comments of the second referee that the the main technical result for the fermions is essentially that in [22], and the philosophy of the calculation is similar, simply with a bit more care taken with the horizon. To make this more explicit we added some more comments. In the introduction below (1.5) (the first mention of the anomalous Luttinger formula) we modify the paragraph from

"An elegant and more general proof was also recently given in [21] for a holographic system with no horizon. Our derivation allows for a horizon and the associated non- trivial widths of fermionic excitations."

to -->

"An elegant and more general proof was also recently given in [22] for a holographic system with no horizon. Our derivation is along similar lines, but also allows for a horizon and the associated nontrivial widths of fermionic excitations."

Also, below equation (3.2) (in the introduction to the fermionic section) we add the line:

"A very similar result was recently obtained in \cite{Sachdev:2011ze} for a system with no horizon; our derivation is slightly more general in that we allow for a horizon and treat carefully the analytic structure and nontrivial quasiparticle widths associated with such a horizon."

Also -- and this is unrelated to the comments of any referee -- we have expanded on one paragraph in the conclusion to be slightly more explicit about how finite-N effects etc. may change our results. The relevant paragraph is on the second column of page 15 and begins "Before further interpreting....". 

Thank you. 

